AdaExploreBench: Benchmarking LLM Agents for Proactive Exploration and Test-time Adaptation in Evolving Environments

Large Language Model (LLM) agents are increasingly deployed in unfamiliar and evolving environments, requiring them to proactively explore, understand, and adapt to environmental dynamics. However, existing benchmarks rarely test whether agents can proactively discover how an environment works and adapt as it evolves. To address this gap, we introduce AdaExploreBench, a benchmark for proactive exploration and test-time adaptation in evolving environments. By instantiating environmental dynamics as hidden rules, AdaExploreBench requires agents to actively acquire evidence and infer the rules. Under implicit rule drift, the latent rule changes without announcement, requiring agents to detect from degraded performance that prior knowledge is stale and re-explore. Experiments on eight leading LLMs show that proactive and adaptive exploration remain challenging: GPT-6 Sol achieves only 61.9% calibrated accuracy, while providing sufficient evidence or removing rule drift improves average performance significantly by close to 10%. These results reveal a critical bottleneck in current LLM agents: they can often reason effectively from informative evidence once it is available, but struggle to actively acquire the right evidence and recognize when previously acquired evidence is no longer valid.

==> latex/0_abstract_ori.tex <==
\begin{abstract}
% % ============== Motivation ================
% Sentence 1: Real-World Challenge. (Why we want to investigate the problem)
% % ============== Gap =======================
% Sentence 2: However, existing work overlooked xxx (gap)
% % ============== Lead-in ===================
% Sentence 3: To address this gap, we introduce \bench{}, a xxx (briefly introduce)
% % ============== Design ====================
% Sentence 4: What did we design to fill in the gap? (In this paper mostly exploration and blocking?)
% % ============== Findings ==================
% Sentence 5: Interesting findings (important takeaways, mostly focus on what, how and why agent fails)
% % ============== Significance ==============
% Sentence 6: Significance "

Large Language Model (LLM) agents are increasingly deployed in partially observable \jiayu{unfamiliar} and evolving environments, requiring them to proactively explore, understand, and adapt to environmental dynamics.
However, existing exploration benchmarks \jiayu{the word ``exploration benchmarks are weird''} are often non-proactive\jiayu{reactive} or non-adaptive \jiayu{static}, and typically task-completion rather than environment-learning. \jiayu{I don't think you should list out all the differences in the abs, the ``task completion'' and ``env learning'' concept is super weird. Just drop it.}
\jiayu{For the last sentence, you should make it sth like: Existing benchmark lack xxx, leaving xxx a blank.}
To address these limitations, we introduce \textbf{\bench{}}, a benchmark for evaluating proactive and adaptive exploration of LLM agents in evolving environments.
\bench{} instantiates environmental dynamics as hidden Rules. 
\jiayu{By instantiating environment dynamics as hidden rules, we provide a dynamic environment for agents to proactively xxx}
Agents proactively \textbf{Probe} \jiayu{the word ``Probe'' is undefined, } by deciding when, what and how much to explore.
When rules change\jiayu{This needs to be named as a some kind of dynamic module, please refer to the complete paper to figure out the name. If there isn't a name for it, you can report.}, they must detect the shift from masked feedback and explore again to adapt.
Experiments on eight leading LLMs show that proactive and adaptive exploration remain challenging: \textit{GPT-6 Sol} achieves only 61.9\% calibrated accuracy, while giving sufficient evidence or removing rule changes significantly improves the performance of the majority of models by 10\% to 20\%.
Together, our results reveal that LLM agents usually learn effectively from given evidence but lag in proactive exploration and test-time adaptation, highlighting key directions for future improvement. \jiayu{The last sentence is not catchy enough, and ``usually learn effectively from given evidence but lag in proactive exploration'', this is weird, I know what you mean, actually you mean that LLMs cannot generate good probes, but can learn effectively from good probes, but the expression is super vague.}
\footnote{\jt{CODE}}
\end{abstract}

==> latex/3_benchmark_construction_ori.tex <==
\section{Benchmark Construction}

\subsection{Task Setup}

\paragraph{Formalization.}
A \textit{task} defines an operational decision setting with a set of input \textit{fields} and an \textit{action set} to choose from.
A \textit{case} is one realization of these fields for which the agent must choose an action.
Each case is represented by a vector of field values.
\textit{factors} are the subset of fields that is relevant to the decision.
The \textit{action set} \(\mathcal{A}=\{a_0,a_1,a_2,a_3\}\) is ordered from the weakest to the strongest intervention level.
A hidden \textit{Rule Function} maps each case to an \textit{intervention score} \(s\in[-1,1]\), where a larger \(s\) indicates a stronger appropriate intervention.
A factor has a \textit{direction} where a positive direction means the intervention score went higher as the factor value gets larger, and vise versa.
A \textit{Utility Function} maps intervention score to the \textit{utilities} of the four actions.
Detailed definitions are provided in Appendix~\ref{app:task_setup_details}. \jeongh{Again, the definitions in Task Setup may help, but we need an example. It seems like the current version of the paper has no explicit example but low-level definition of tasks and how they are evaluated which sounds a bit vague.}

\paragraph{Rule Families.}
We consider four rule families that represent common ways of combining multiple attributes in decision making.
Prior work broadly distinguishes \textit{compensatory} rules, where evidence from different attributes can offset each other, from \textit{non-compensatory} rules, where decisions depend on thresholds or attribute priorities
\citep{einhorn1970nonlinear,payne1993adaptive}.
We instantiate one representative family for each combination strategy.
\textit{Additive} rules aggregate evidence from all relevant fields; 
\textit{conjunctive} rules require \textit{all} conditions to be satisfied;
\textit{disjunctive} rules require only \textit{any} one condition;
and \textit{lexicographic} rules examine fields in a \textit{priority order}.
Detailed descriptions and illustrations are provided in Appendix~\ref{app:task_setup_details}.

\paragraph{Rule and Utility Functions.}
The Rule Function determines the latent decision rule that governs how the factors interact.
It normalizes each factor to \([-1,1]\), combines them into raw evidence through one of the four rule families, and maps the evidence to the intervention score \(s\) via a monotonic calibration, so that each family induces a distinct mode of factor interaction on a common scale.
The Utility Function, by contrast, is a purely mechanistic component and does not shape the latent rule.
It only maps the continuous score into rewards over the four discrete actions.
Each action is tied to a fixed intervention level, and its reward is higher when this level is closer to the score, so the notion of intervention level semantically aligns the discrete action space with the continuous score.
The exact definitions, calibration procedure, and utility construction are given in Appendix~\ref{app:task_setup_details}.

\subsection{Data Generation}

\paragraph{Formalization.} 
We construct benchmark data at the episode level.
An \textit{episode} is an instantiated \textit{task} that serves as a self-contained unit of evaluation, defined as \(\mathcal{E}=(\sigma,\mathcal{F}_{\mathcal{E}},\mathcal{R}_{\mathcal{E}},\mathcal{B}_{\mathcal{E}},\Delta_{\mathcal{E}})\), where \(\sigma\) denotes the \textit{task} metadata, \(\mathcal{F}_{\mathcal{E}}\) the selected observable fields, \(\mathcal{R}_{\mathcal{E}}\) the instantiated hidden rule(s) from \(R_\theta\), \(\mathcal{B}_{\mathcal{E}}\) the evaluation cases organized into batches, and \(\Delta_{\mathcal{E}}\) the rule transition in dynamic settings (empty for static episodes).
We generate episodes through a two-stage process.
First, we construct reusable semantic templates \(\mathcal{T}=(\sigma,\mathcal{F},\Gamma,\Lambda)\), where \(\sigma\) specifies the scenario metadata, \(\mathcal{F}\) the field catalog, \(\Gamma\) the cross-field feasibility constraints, and \(\Lambda\) the rule-related semantic specifications.
Second, we construct episodes from these templates by enumerating field configurations, instantiating hidden rules, and sampling evaluation cases after validity filtering.

\paragraph{Semantic Template Construction.} 
Template \(\mathcal{T}\) is constructed through a multi-step LLM-assisted synthesis process guided by a predefined schema \jeongh{How did you validate the multi-step LLM-assisted synthesis process? Were there any validation measure to assess the correctness of these steps?}.
The process can be summarized as 
(i) establishing task metadata \(\sigma\), including the scenario description, agent role, and task-instantiated action space \(\mathcal{A}\), (ii) generating the field catalog \(\mathcal{F}\), including field definitions, semantic parameters, and value distributions, 
(iii) constructing cross-field feasibility constraints \(\Gamma\) governing valid field combinations, and 
(iv) constructing rule-related specifications \(\Lambda\), including rule-family applicability, rule-specific relations, and admissible \dynamic{}.
For our evaluation dataset, task metadata \(\sigma\) is fixed using predefined blueprints to ensure consistent task settings.
Generated components undergo programmatic validation and LLM-based semantic auditing before being assembled into the template. Detailed construction procedures are provided in Appendix~\ref{app:data}.

\paragraph{Episode Generation.} 
For each accepted template \(\mathcal{T}\), we enumerate field configurations \(\mathcal{F}_{\mathcal{E}}\subseteq\mathcal{F}\) and instantiate the corresponding latent rule specifications \(\mathcal{R}_{\mathcal{E}}\), retaining those that satisfy three complementary validity criteria:
 
\begin{itemize}
    \item \textbf{Structural Validity.} The selected fields comprise factors indexed by \(\mathcal{I}\) and additional distractor fields, admit a non-empty feasible case space under \(\Gamma\), and satisfy the rule-family applicability constraints in \(\Lambda\). For dynamic episodes, the rule transition \(\Delta_{\mathcal{E}}\) additionally satisfies the admissible transition constraints in \(\Lambda\).
    \item \textbf{Numerical Validity.} The instantiated rule \(\mathcal{R}_{\mathcal{E}}\) induces non-degenerate distributions of optimal actions over the feasible case population. For dynamic episodes, the \dynamic{} induces meaningful yet moderate changes in optimal-action assignments.
    \item \textbf{Semantic Plausibility.} The selected field configuration \(\mathcal{F}_{\mathcal{E}}\) and, for dynamic episodes, the \dynamic{} are semantically consistent with the task scenario.
\end{itemize}

\noindent Given \(\mathcal{F}_{\mathcal{E}}\), \(\mathcal{R}_{\mathcal{E}}\) (and \(\Delta_{\mathcal{E}}\) for dynamic episodes), we sample evaluation cases \(\mathbf{x}\in\mathcal{X}\) from the field distributions specified by \(\mathcal{F}\), subject to \(\Gamma\) and additional transition-aware sampling for dynamic episodes. We compute the action utilities \(\mathcal{U}(R_\theta(\mathbf{x}))\), organize the cases into evaluation batches \(\mathcal{B}_{\mathcal{E}}\), and assemble these batches with the other episode components to form the complete episode \(\mathcal{E}\).
For the evaluation dataset, we additionally conduct a multi-dimensional review and select the highest-scoring qualified episodes, retaining 256 of 384 episodes for the final benchmark. Detailed episode instantiation procedures, algorithms, and review prompts are provided in Appendix~\ref{app:data}.



\subsection{Runtime Protocol}
\paragraph{Definitions.} An \textit{episode} refers to one evaluation instance.
The agent \textit{probes} by filling in values of input fields and get the utilities of all actions for the case.
A \textit{batch} refers to a group of cases.
An agent \textit{complete} an evaluation batch by submitting action choices for each case in the batch.
A \textit{probe batch} means the cases are suggested by the agent, and a \textit{evaluation batch} means the cases are provided by the environment for the agent to complete.

\paragraph{Information Disclosure.}
The agent receives the task description, the input fields and their ranges, the action set $\mathcal{A}$, definitions of four rule families, and the available interaction tools.
It is also informed that the environment follows a latent rule in one of the four families, and it may change during interaction.
The environment shows a current state including cumulative utility gained and usable tools before each interaction.
The actual rule family, factors, rule thresholds, and the occurrence and timing of \dynamic{} remain hidden.

\paragraph{Tools for Interaction.}
Each episode proceeds through evaluation batches.
Before each batch is revealed, the agent enters an exploration window in which it may probe or proceed without probing.
The available interaction tools are as follows:

\begin{itemize}
    \item \texttt{probe\_batch} allows the agent to query one or more cases by specifying their input field values. It returns the utility of all actions for each case.
    \item \texttt{request\_next\_batch} ends the exploration window and jumps to the next evaluation batch.
    \item \texttt{submit\_action\_batch} allows the agent to submit one action for each case in the current evaluation batch. It returns the utility gain of the selected action and also other actions.

    \item \texttt{calculator} supports numerical calculations during rule inference and action selection.
\end{itemize}

\paragraph{Masking Evaluation Batch.}
By default, evaluation cases are visible only while the current batch is being solved.
Once the batch is submitted, the case values and selected actions are removed from subsequent context.
Only utility outcomes are left in the context.
In contrast, probe observations remain available in the interaction history.
This design prevents the environment from leaking evidence through evaluation batches, while still allowing their realized utilities to provide performance feedback for the agent to detect a possible \dynamic{}.

\paragraph{\Dynamic{} and the Detection.}
\textit{\dynamic{}} is the dynamic event that may occurs immediately after a completed evaluation batch.
The rule remains within the same family but alters a factor and reverse a factor direction.
The interaction protocol remains unchanged.
The agent must detect from evaluation and probe outcomes and adapt its subsequent exploration accordingly.

\paragraph{Auxiliary Assessment.}
We use out-of-band auxiliary assessments to directly evaluate whether the agent has identified the factors, their directional effects, and the hidden rule drift. For dynamic settings, assessments are collected immediately before the rule change and at the end of an episode. For stationary settings, a single assessment is collected at the end of the episode. These assessments are not added to the agent's subsequent context.

\paragraph{Detailed Settings.}
All detailed settings, including:
(1) Error Handling. 
(2) Number and size of evaluation batches.
(3) Detailed prompts.
(4) \dynamic{} timing.
are prvided in Appendix~\ref{app:runtime_settings}.
